Representation Magnitude has a Liability to Privacy Vulnerability

The privacy-preserving approaches to machine learning (ML) models have made substantial progress in recent years. However, it is still opaque in which circumstances and conditions the model becomes privacy-vulnerable, leading to a challenge for ML models to maintain both performance and privacy. In this paper, we first explore the disparity between member and non-member data in the representation of models under common training frameworks. We identify how the representation magnitude disparity correlates with privacy vulnerability and address how this correlation impacts privacy vulnerability. Based on the observations, we propose Saturn Ring Classifier Module (SRCM), a plug-in model-level solution to mitigate membership privacy leakage. Through a confined yet effective representation space, our approach ameliorates models' privacy vulnerability while maintaining generalizability. The code of this work can be found here: \url{https://github.com/JEKimLab/AIES2024_SRCM}

==> fig_tex/fig_acc_auc.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/acc_auc_c10.pdf}
        \caption{Performance of defenses against different adaptive MIAs (ResNet18, CIFAR-10). Being lower and more rightward is better.}
        \label{fig:acc_mia_c10}
     \end{subfigure}
     \begin{subfigure}[]{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/acc_auc_c100.pdf}
        \caption{Performance of defenses against different adaptive MIAs (ResNet18, CIFAR-100). Being lower and more rightward is better.}
    \label{fig:acc_mia_c100}
     \end{subfigure}
     \begin{subfigure}[]{0.95\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/acc_auc_p100.pdf}
        \caption{Performance of defenses against different adaptive MIAs (MLP, Purchase100). Being lower and more rightward is better.}
    \label{fig:acc_mia_p100}
     \end{subfigure}
     %\vspace*{-6.mm}
\caption{Performance of defenses against different adaptive MIAs among different datasets.}
\label{fig:acc_mia}
\end{figure*}

==> fig_tex/fig_distribution.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=.79\linewidth]{figs/eg_fig3.png}
\caption{Exp Fig 2 Example, want to show some distribution thing here.}
\label{fig:distribution_w_various_conf}
\end{figure*}

==> fig_tex/fig_hyper-parameters.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=1.\linewidth]{figs/eg_fig_hyper-parameters.png}
\caption{Exp Fig Example, want to show some changes with hyper-parameters.}
\label{fig:helight}
\end{figure}

==> fig_tex/fig_index.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=1.\linewidth]{figs/eg_fig1.png}
\caption{Exp Fig 1 Example, want to show some training tech w/ and w/o our module.}
\label{fig:helight}
\end{figure}

==> sec/NotUsed_0_abstract.tex <==
% \begin{abstract}

% The privacy-preserving technology for machine learning (ML) models has made substantial progress in recent years.
% However, it is still indeterministic in which circumstances the model becomes privacy-vulnerable, leading to difficulty for ML models to maintain both performance and privacy.
% In this paper, we first explore the disparity in the representation of models under common training frameworks between member and non-member data. Then, we show how the representation magnitude disparity correlates with privacy vulnerability and study how this association impacts the ease of privacy leakage. Finally, based on our observations, we propose Saturn Ring Classifier Module (SRCM), a plug-in model-level solution to mitigate membership privacy leakage. Via a confined yet effective representation space, our approach can ameliorate models' privacy vulnerability while maintaining generalizability.
% \end{abstract}

==> tabs/res_cmp_srcm_1.tex <==
%\renewcommand\arraystretch{0.8}
\begin{table}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{|l|l|c|c|c|c|c|c|c|}
    %%%%%%%%%%%%%%%%%%%%% Top Line %%%%%%%%%%%%%%%%%%%%%
    \hline
    Dataset & Models \& Approach & Train (\%) & Test (\%) & NN (\%) & Entr. (\%) & M-Entr. (\%) & Grad-$x$ & Grad-$w$ (\%)\\
    %%%%%%%%%%%%%%%%%%%%% Mid Line %%%%%%%%%%%%%%%%%%%%%
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%% MobileNet %%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hline
    & MobileNetV3 (large)     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    & + CondConv ($4\times$)              & - & - & - & - & - & - & - \\
    & + CondConv ($8\times$)              & - & - & - & - & - & - & - \\
    & + DyConv ($4\times$)                & - & - & - & - & - & - & - \\
    & + DyConv ($8\times$)                & - & - & - & - & - & - & - \\
    & + ODConv ($4\times$)                & - & - & - & - & - & - & - \\
    & + ODConv ($8\times$)                & - & - & - & - & - & - & - \\
    & + XXConv ($8\times$, Ours)          & - & - & - & - & - & - & - \\
    \hline
    & MobileNetV1 ($1.0\times$ width)     & - & - & - & - & - & - & - \\
    & + CondConv ($4\times$)              & - & - & - & - & - & - & - \\
    & + CondConv ($8\times$)              & - & - & - & - & - & - & - \\
    & + DyConv ($8\times$)                & - & - & - & - & - & - & - \\
    & + ODConv ($8\times$)                & - & - & - & - & - & - & - \\
    & + XXConv ($8\times$, Ours)          & - & - & - & - & - & - & - \\
    \hline

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%% PramidNet %%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    %%%%%%%%%%%%%%%%%%%%% Bottom Line %%%%%%%%%%%%%%%%%%
    \hline
  \end{tabular}
  }
  \caption{Results comparison on the ImageNet. %using different convolution OPs and backbones.
  %MobileNetV1 $(1.0\times, 0.75\times, 0.5\times)$ backbones and additive PyramidNet backbones with 110 depth and $(48, 84, 270)$ widening factors.
  }
  \label{tab:res_cifar100}

\end{table}

==> tabs/res_cmp_srcm_2.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\large
\begin{tabular}{llcccccc|ccccc|ccccc}
\toprule
& & &
\multicolumn{5}{c}{\large{\textbf{CIFAR-10}}} & 
\multicolumn{5}{c}{\large{\textbf{CIFAR-100}}} & 
\multicolumn{5}{c}{\large{\textbf{Tiny ImageNet}}} \\   
\cmidrule(lr){4-8} \cmidrule(lr){9-13} \cmidrule(lr){14-18}
\large{\textbf{Model}} & \large{\textbf{Train Tech.}} & \large{\textbf{W/ SRCM}}  
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}} 
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}}
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}}
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% MobileNetV3 (Small) %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{11}{*}{MobileNetV3} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
- (Small) & & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% MobileNetV3 (Large) %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{MobileNetV3} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
- (Large) & & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% ResNet18 %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{ResNet18} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 99.99 & 58.05 & 81.14 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 92.86 & 57.90 & 50.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 94.24 & 47.94 & 69.50 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 95.22 & 59.19 & 50.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% ResNet18 %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{ResNet18} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-18}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-18}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%\midrule
%\midrule
%%%%%%%%%%%%%% details
\bottomrule
\end{tabular}
} % \resizebox
\caption{
    \textbf{Evaluations on CIFAR-, 10, 100, and Tiny ImageNet} -- `Train' and `Test' stand for training and testing accuracy. 
} % \caption
\label{tab:exp_ac_res_3}%
\end{table*}

==> tabs/res_cmp_srcm_3.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\large
\begin{tabular}{llcccccccc|ccccccc|ccccccc}
\toprule
& & &
\multicolumn{7}{c}{\large{\textbf{CIFAR-10}}} & 
\multicolumn{7}{c}{\large{\textbf{CIFAR-100}}} & 
\multicolumn{7}{c}{\large{\textbf{Tiny ImageNet}}} \\   
\cmidrule(lr){4-10} \cmidrule(lr){11-17} \cmidrule(lr){18-24}
\large{\textbf{Model}} & \large{\textbf{Train Tech.}} & \large{\textbf{W/ SRCM}}  
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}} & \large{\textbf{MIAs 4}} & \large{\textbf{MIAs 5}} 
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}} & \large{\textbf{MIAs 4}} & \large{\textbf{MIAs 5}} 
& \large{\textbf{Train}} & \large{\textbf{Test}} & \large{\textbf{MIAs 1}} & \large{\textbf{MIAs 2}} & \large{\textbf{MIAs 3}} & \large{\textbf{MIAs 4}} & \large{\textbf{MIAs 5}} 
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% MobileNetV3 (Large) %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{MobileNetV3} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
- (Large) & & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% ResNet18 %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{ResNet18} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 99.99 & 58.05 & 81.14 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 92.86 & 57.90 & 50.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 94.24 & 47.94 & 69.50 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 95.22 & 59.19 & 50.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% ResNet18 %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multirow{11}{*}{ResNet18} 
& \multirow{2.5}{*}{CE} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{AdvReg} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{RelaxLoss} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){2-24}
& \multirow{2.5}{*}{Approach 3} & \ding{55}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\ \cmidrule(lr){3-24}
& & \ding{51}
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
& 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00
\\
%\midrule
%\midrule
%%%%%%%%%%%%%% details
\bottomrule
\end{tabular}
} % \resizebox
\caption{
    \textbf{Evaluations on CIFAR-10, -100, and Tiny ImageNet} -- `Train' and `Test' stand for training and testing accuracy, respectively. 
} % \caption
\label{tab:exp_ac_res_3}%
\end{table*}

==> tabs/result.tex <==
{
\setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{.9} % Default value: 1
\begin{table*}
  \centering
  \resizebox{.9\linewidth}{!}{
  \begin{tabular}{|c|c|c|c|l|l|l|l|l|}
    %%%%%%%%%%%%%%%%%%%%% Top Line %%%%%%%%%%%%%%%%%%%%
    \hline
    \textbf{Datasets} & \textbf{Models} & \textbf{Train Tech.} & 
    \textbf{W/ SRCM (Ours)} & \textbf{Trian Acc. (\%)} & \textbf{Test Acc. (\%)} & 
    \textbf{NN-Based (\%)} & \textbf{MIAs 2 (\%)} & \textbf{MIAs 3 (\%)} \\
    %%%%%%%%%%%%%%%%%%%%% Mid Line %%%%%%%%%%%%%%%%%%%%
    %\cmidrule{2-5}
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%% CIFAR-10 %%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hline
    \multirow{4}{*}{CIFAR-10}
    %%%%%%%%%%% VGG
    & \multirow{4}{*}{VGG11}
     & \multirow{2}{*}{CE (Baseline)} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    \cline{3-9}
    && \multirow{2}{*}{AdvReg} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    \cline{3-9}
    && \multirow{2}{*}{RelaxLoss} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    \cline{3-9}
    && \multirow{2}{*}{approach 3} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    %%%%%%%%%%% ResNet
    \cline{2-9}
    & \multirow{4}{*}{ResNet18} 
     & \multirow{2}{*}{CE (Baseline)} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    \cline{3-9}
    && \multirow{2}{*}{AdvReg} 
      & \ding{55} & - & - & - & - & - \\
    &&& \ding{51} & - & - & - & - & - \\
    \cline{3-9}
    && \multirow{2}{*}{RelaxLoss} 
      & \ding{55} & - & - & - & - & - \\
    &&& \ding{51} & - & - & - & - & - \\
    \cline{3-9}
    && \multirow{2}{*}{approach 3} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%% CIFAR-100 %%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hline
    \multirow{4}{*}{CIFAR-100}
    & \multirow{4}{*}{ResNet18} 
     & \multirow{2}{*}{CE (Baseline)} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    \cline{3-9}
    && \multirow{2}{*}{AdvReg} 
      & \ding{55} & - & - & - & - & - \\
    &&& \ding{51} & - & - & - & - & - \\
    \cline{3-9}
    && \multirow{2}{*}{RelaxLoss} 
      & \ding{55} & - & - & - & - & - \\
    &&& \ding{51} & - & - & - & - & - \\
    \cline{3-9}
    && \multirow{2}{*}{approach 3} 
      & \ding{55} & -  & -  & -  & -  & - \\
    &&& \ding{51} & -  & -  & -  & -  & - \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%% TinyImageNet %%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%% Bottom Line %%%%%%%%%%%%%%%%%%%%%
    \hline
  \end{tabular}
  }
  \caption{Results comparison among multiple image datasets. Data augmentations are applied to CIFAR-100 and TinyImageNet.
  }
  \label{tab:res_main}
\end{table*}
}
